Can A User Anticipate What Her Followers Want?

Whenever a social media user decides to share a story, she is typically pleased to receive likes, comments, shares, or, more generally, feedback from her followers. As a result, she may feel compelled to use the feedback she receives to (re-)estimate her followers' preferences and decides which stories to share next to receive more (positive) feedback. Under which conditions can she succeed? In this work, we first look into this problem from a theoretical perspective and then provide a set of practical algorithms to identify and characterize such behavior in social media. More specifically, we address the above problem from the viewpoint of sequential decision making and utility maximization. For a wide variety of utility functions, we first show that, to succeed, a user needs to actively trade off exploitation-- sharing stories which lead to more (positive) feedback--and exploration-- sharing stories to learn about her followers' preferences. However, exploration is not necessary if a user utilizes the feedback her followers provide to other users in addition to the feedback she receives. Then, we develop a utility estimation framework for observation data, which relies on statistical hypothesis testing to determine whether a user utilizes the feedback she receives from each of her followers to decide what to post next. Experiments on synthetic data illustrate our theoretical findings and show that our estimation framework is able to accurately recover users' underlying utility functions. Experiments on several real datasets gathered from Twitter and Reddit reveal that up to 82% (43%) of the Twitter (Reddit) users in our datasets do use the feedback they receive to decide what to post next.

==> 11related.tex <==
Our work is conceptually related with several fields of research, viz. (i) revealed preferences, (ii) Empirical analysis of user' behavior in social media,
(iii) regret analysis of bandit problems, and (iii) behavior shaping in social networks. We will briefly review the related works in these are separately.

\xhdr{Revealed preferences} 
Reveal preference theory, pioneered by Samuelson~\cite{samuelson1948consumption}, is a well-established economic theory of analyzing choices made by agents. It assumes
that an agent will decide to buy a bundle of goods, which she most prefers among all and is able to afford, according to some concave increasing utility function. Since then,
research on revealed preference analysis predominantly focus to design a realistic model for an agent's utility function~\cite{koo1963empirical,mas1977recoverability,afriat1967construction}. 
%
More recently, an extensive line of work has exploited statistical learning theory to design efficient algorithms for estimating the utility function from revealed preference data, and derive
sample complexity for these algorithms for a class of utility functions~\cite{beigman2006learning,zadimoghaddam2012efficiently,echenique2011revealed,balcan2014learning}. However, these works
differ from our approach in two key aspects: (i) these models are specifically designed to explain a customer's behavior during purchasing goods--- they cannot be easily extended to explain the posting behavior of a broadcaster
in online social networks; (ii) their settings for utility maximization assume complete knowledge of all model parameters, and furthermore, their maximization strategies do not provide guarantee when the unknown parameters
are substituted with their estimates.

\xhdr{Empirical studies of user's behavior in social media} Empirical studies on analyzing users' behavior in social media, strongly suggest that the feedbacks in different forms carry social value
which motivates people to posts~\cite{burke2013using,burke2014growing,ellison2014cultivating,gray2013wants,burke2010social,grinberg2016changes,grinberg2017understanding,cheng2014community}. 
To that aim, some of these works draw on existing principles on psychology to design hypotheses about the posting behavior on people in social media. In particular,
Grinberg \emph{et al}~\cite{grinberg2016changes} discusses the behavior changes in user engagement before and after posting to Facebook. Furthermore, in a following work~\cite{grinberg2017understanding}, 
they have built on Expectation Violation Theory~\cite{burgoon1978communication,burgoon1993effects} to comprehensively examine the factors associated with feedback expectations of users after posting in Facebook. 
In a similar note, Cheng \emph{et al}
relied on operant conditioning framework~\cite{skinner1988preface} for investigating the effects of positive and negative feedbacks on the quality of future posts. Moreover, they observed that, the users
who receive no feedback, are likely to leave the online platform. However, these empirical studies only analyzed the aggregated behavior of the entire population, not the individual behavior.
Furthermore, they neither offer any modeling framework for the user-feedback interaction, nor any strategy to attract more positive evaluations by exploiting past feedbacks.

\xhdr{Shaping people's behavior in online social networks} Very recently, there has been a flurry of research on designing algorithms to control people's posting behavior in online social media~\cite{redqueen17wsdm,smart16,Farajtabar2014,jmlr}.
More specifically, these works rely on maximizing quality metrics \emph{e.g.} visibility, total number of activities, etc., by means of online adaptive interventions. However,
these works have two major limitations that constrain their applicability in the current setting: (i) they assume complete knowledge of all the parameters in their quality metrics;
(ii) their quality metrics are very difficult to learn from real data.

\xhdr{Regret analysis} The proof techniques employed to derive the regret bounds for the our algorithm is related to the methods for deriving bounds in bandit problems and
reinforcement learning~\cite{tspaper,auer2007logarithmic,jaksch2010near,agrawal2013thompson}. However, our techniques
are different from others in two key aspects: (i) our method allows a broadcaster to exploit additional information from the feedbacks of her followers to  others' messages for estimating the unknown preferences, whereas, a
traditional bandit setting only allows a broadcaster to use the feedback to her own messages; (ii) our proof techniques generalize over a number of neighbors, whereas the traditional bandit setting helps us to derive regrets
only for one neighbor.


